Hadronic production of squark-squark pairs: The electroweak contributions

We compute the electroweak (EW) contributions to squark--squark pair production processes at the LHC within the framework of the Minimal Supersymmetric Standard Model (MSSM). Both tree-level EW contributions, of O(alpha_s alpha + alpha^2), and next-to-leading order (NLO) EW corrections, of O(alpha_s^2 alpha), are calculated. Depending on the flavor and chirality of the produced quarks, many interferences between EW-mediated and QCD-mediated diagrams give non-zero contributions at tree-level and NLO. We discuss the computational techniques and present an extensive numerical analysis for inclusive squark--squark production as well as for subsets and single processes. While the tree-level EW contributions to the integrated cross sections can reach the 20% level, the NLO EW corrections typically lower the LO prediction by a few percent.

==> feynman/table2.tex <==
\TABULAR[h]{c|llr}{
  subprocess & flavor multiplicity & chirality multiplicity & sum \\
  \hline
  \parbox{2.5cm}{$qq \rightarrow \tilde q_a \tilde q_b$}
  & 4 (uu, dd, cc, ss) & 3 (LL, RR, LR) & 12\\[15pt]
  \parbox{2.5cm}{{$qq^{\prime} \rightarrow \tilde q_a
      \tilde q_b^{\prime}$}\\{\footnotesize same doublet}}
  & 2 (ud, cs) & 4 (LL, RR, LR, RL) & 8\\[15pt]
  \parbox{2.5cm}{$qq^{\prime} \rightarrow \tilde q_a
    \tilde q_b^{\prime}$\\{\footnotesize different doublet}}
     & 4 (uc, us, dc, ds) & 4 (LL, RR, LR, RL) & 16\\[10pt]
  \hline
  &&& $\sum 36$
}
{Different channels contributing to squark--squark
    production. The capital letters L (left-handed) and R (right-handed)
    label the chirality of the first and second squark.
\label{tab_multiplicity}}


==> feynman/treelevel.tex <==

\unitlength=0.2bp%
%1
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FALabel(5.0774,15.8181)[b]{$q$}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{1}
\FALabel(3.36888,4.18457)[t]{$q^{\prime}$}
\FAProp(20.,15.)(10.,14.)(0.,){/ScalarDash}{-1}
\FALabel(14.9226,15.8181)[b]{$\tilde q_\alpha$}
\FAProp(20.,5.)(10.,6.)(0.,){/ScalarDash}{-1}
\FALabel(16.6311,4.18457)[t]{$\tilde q^{\prime}_\beta$}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{0}
\FALabel(9.18,10.)[r]{$\tilde g$}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
\end{feynartspicture}
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FALabel(5.0774,15.8181)[b]{$q$}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{1}
\FALabel(3.36888,4.18457)[t]{$q^{\prime}$}
\FAProp(20.,15.)(10.,14.)(0.,){/ScalarDash}{-1}
\FALabel(14.9226,15.8181)[b]{$\tilde q_\alpha$}
\FAProp(20.,5.)(10.,6.)(0.,){/ScalarDash}{-1}
\FALabel(16.6311,4.18457)[t]{$\tilde q^{\prime}_\beta$}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{0}
\FALabel(9.18,10.)[r]{$\tilde \chi_m^0$}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
\end{feynartspicture}
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FALabel(5.0774,15.8181)[b]{$q$}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{1}
\FALabel(3.36888,4.18457)[t]{$q^{\prime}$}
\FAProp(20.,15.)(10.,6.)(0.,){/ScalarDash}{-1}
\FALabel(14.9226,15.8181)[b]{$\tilde q_\alpha$}
\FAProp(20.,5.)(10.,14.)(0.,){/ScalarDash}{-1}
\FALabel(16.6311,4.18457)[t]{$\tilde q^{\prime}_\beta$}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{-1}
\FALabel(9.03,10.)[r]{$\tilde \chi_m$}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
\end{feynartspicture}\\
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FALabel(5.0774,15.8181)[b]{$u$}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{1}
\FALabel(3.36888,4.18457)[t]{$s$}
\FAProp(20.,15.)(10.,14.)(0.,){/ScalarDash}{-1}
\FALabel(14.9226,15.8181)[b]{$\tilde c_\alpha$}
\FAProp(20.,5.)(10.,6.)(0.,){/ScalarDash}{-1}
\FALabel(16.6311,4.18457)[t]{$\tilde d_\beta$}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{0}
\FALabel(9.18,10.)[r]{$\tilde \chi_m$}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
\end{feynartspicture}
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FALabel(5.0774,15.8181)[b]{$c$}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{1}
\FALabel(3.36888,4.18457)[t]{$d$}
\FAProp(20.,15.)(10.,14.)(0.,){/ScalarDash}{-1}
\FALabel(14.9226,15.8181)[b]{$\tilde u_\alpha$}
\FAProp(20.,5.)(10.,6.)(0.,){/ScalarDash}{-1}
\FALabel(16.6311,4.18457)[t]{$\tilde s_\beta$}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{0}
\FALabel(9.18,10.)[r]{$\tilde \chi_m$}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
\end{feynartspicture}
